CHEF: A Pilot Chinese Dataset for Evidence-Based Fact-Checking

The explosion of misinformation spreading in the media ecosystem urges for automated fact-checking. While misinformation spans both geographic and linguistic boundaries, most work in the field has focused on English. Datasets and tools available in other languages, such as Chinese, are limited. In order to bridge this gap, we construct CHEF, the first CHinese Evidence-based Fact-checking dataset of 10K real-world claims. The dataset covers multiple domains, ranging from politics to public health, and provides annotated evidence retrieved from the Internet. Further, we develop established baselines and a novel approach that is able to model the evidence retrieval as a latent variable, allowing jointly training with the veracity prediction model in an end-to-end fashion. Extensive experiments show that CHEF will provide a challenging testbed for the development of fact-checking systems designed to retrieve and reason over non-English claims.

==> tables/case.tex <==
\begin{CJK*}{UTF8}{gbsn}
\begin{table*}[t]
\label{Case study}
\centering
\scalebox{0.75}{
\begin{tabularx}{21cm}{XX}
\toprule
\textbf{Claim 1}: 喝纯净水会缺钙。Drinking pure water will lack calcium. \textcolor{orange}{REF}\\
\midrule
\textbf{Sem}: 喝水如此重要，不少新闻也盯上了纯净水。关于纯净水，一直有很多说法。一直喝纯净水会缺微量元素对身体不好，每天喝4升水会导致中毒。Drinking water is so important that many news have focused on pure water. There have been many sayings about pure water. Drinking pure water for a long time will be deficient in trace elements, which is bad for the body. Drinking 4 liters of water a day will cause poisoning. \textcolor{blue}{NEI}\\
\midrule
\textbf{JG}: 人体能够从水中获得的微量元素其实很少。 The human body can obtain very few trace elements from water. \textcolor{blue}{NEI}\\
\midrule
\textbf{JS}: 喝水并不是补充钙质的主要途径，而喝纯净水也不会对钙的吸收有所影响。所以喝水导致缺钙，说法并不科学。Drinking water is not the main way to supplement calcium, and drinking pure water will not affect calcium absorption. Therefore, it is not scientific to say that drinking water causes calcium deficiency. \textcolor{orange}{REF} \\
\midrule
\textbf{Gold}: 人体钙元素的来源主要是膳食提供，机体是否缺钙与多种因素有关。用喝水来判定是否补充了大量钙的说法并不科学。The source of calcium in the human body is mainly provided by diet. Whether the body is lack of calcium is related to many factors. It is not scientific to use drinking water to determine whether a large amount of calcium has been absorbed. \textcolor{orange}{REF} \\
\midrule
\midrule
\textbf{Claim 2}: 蚊蝇可以传播新冠病毒。Mosquitoes and flies can transmit the COVID-19. \textcolor{orange}{REF}\\
\midrule
\textbf{Sem}: 蚊蝇是否会传播新型冠状病毒？蚊蝇叮咬是否会传播新冠病毒？夏季已至，蚊蝇是否会传播新冠病毒也为外界所关注。新冠病毒可能污染一些食材，但不太可能通过食物传播.食物中存在蚊蝇的卵可能导致疫病的传播。Will mosquitoes and flies spread the COVID-19? Will the bite of mosquitoes and flies transmit the COVID-19? Summer is here, and whether mosquitoes and flies can spread the COVID-19 is also of concern to everyone. The COVID-19 may contaminate some food materials, but it is unlikely to be spread through food. The presence of mosquitoes and flies eggs in the food may cause the spread of the disease. \textcolor{blue}{NEI}\\
\midrule
\textbf{JG}: 尽管不传播新冠病毒，但蚊子仍然是一种害虫，而且是地球上最危险的动物之一。Although it does not spread the COVID-19, the mosquito is still a pest and one of the most dangerous animals on the planet. \textcolor{orange}{REF}\\
\midrule
\textbf{JS}: 从掌握的流行病学证据来看，全球目前没有发现因为蚊蝇等媒介生物导致人感染新冠病毒的报道。Judging from the available epidemiological evidence, there are currently no reports of human infection with the COVID-19 due to vectors such as mosquitoes and flies. \textcolor{orange}{REF} \\
\midrule
\textbf{Gold}: 根据目前研究，蚊蝇不具备传播新冠病毒的生物学基础。According to current research, mosquitoes and flies do not have the biological basis for spreading the COVID-19. \textcolor{orange}{REF} \\

\bottomrule
\end{tabularx}}
\vspace{-2mm}
\caption{Case study of the joint system. The evidence extracted by pipeline and joint systems based on the given claim is listed. The gold label of the claim and the veracity label based on the extracted evidence is highlighted.}
\label{tab:case_study}
% \vspace{-4mm}
\end{table*}
\end{CJK*}

==> tables/error.tex <==
\begin{CJK*}{UTF8}{gbsn}
\begin{table*}[t]
\label{Case study}
\centering
\scalebox{0.75}{
\begin{tabularx}{21cm}{XX}
\toprule
\textbf{Claim 1}: 频繁查询征信不会影响借款。Frequent inquiries about credit investigation will not affect borrowing from the bank. \textcolor{blue}{NEI}\\
\midrule
\textbf{JS}: 个人征信报告因贷款、信用卡审批等原因被不同机构多次查询，但征信报告却显示该段时间内用户没有成功获批新贷款或成功申请到信用卡，那么，银行有理由推测该用户财务状况不佳，从而拒绝用户的申贷请求。The personal credit report has been queried many times by different agencies due to loan, credit card approval and other reasons, but the credit report shows that the user has not successfully obtained a new loan or successfully applied for a credit card during this period, then, the bank has reason to speculate that the user's financial status is poor, and thus rejects the user's loan application request. \textcolor{orange}{REF} \\
\midrule
\textbf{Gold}: 据银行业务人士透露，频繁查询征信记录对于客户信用评估会造成一定影响，一般情况下，银行未经客户许可不会私查征信，通常会在贷前、贷中及贷后监管环节进行查询，但不会过于频繁；不过具体操作中，确实存在一些操作不太合规的情况。一般来说，一段时间内，个人征信报告因贷款、信用卡审批等原因被不同机构多次查询，但征信报告却显示该段时间内用户没有成功获批新贷款或成功申请到信用卡，那么，银行有理由推测该用户财务状况不佳，从而拒绝用户的申贷请求。According to bankers, frequent checking of credit records will have a certain impact on customer credit evaluation. Under normal circumstances, banks will not privately inquire credit without the customer’s permission. Inquiries are usually conducted in the pre-loan, during and after-loan supervision links, but not too frequently. However, in specific operations, there are indeed some operations that are not compliant. Generally speaking, within a period of time, personal credit report has been queried many times by different agencies due to loan, credit card approval and other reasons, but the credit report shows that the user has not successfully obtained a new loan or successfully applied for a credit card within this period of time, then, the bank has reason to speculate that the user's financial status is poor, and thus rejects the user's loan application request. \textcolor{blue}{NEI}\\
\midrule
\midrule
\textbf{Claim 2}: 2019年，杭州有银行悄悄调整了房贷政策，父母和子女两代人可接力还款，规定房屋按揭贷款最长可贷到80周岁。In 2019, a bank in Hangzhou quietly adjusted its mortgage policy. Parents and children of two generations can relay the loan, and it is stipulated that the mortgage loan can be loaned up to 80 years of age. \textcolor{orange}{REF}\\
\midrule
\textbf{JS}: 该行通过官方微博声明回应称，该行接力贷产品，是指具有完全民事行为能力的父亲(或母亲)与一名具有完全民事行为能力的儿子(或女儿)两者作为共同借款人，向银行申请的个人住房贷款。该产品通过增加子女作为共同借款人，并以子女年龄测算贷款期限(年龄+贷款期限不超过70岁)，有效满足了家庭成员共同参与的合理住房贷款需求，有效降低了客户还款压力，不存在年龄超过70岁还能贷款的情形，符合监管的要求。The bank responded in an official Weibo statement that the bank’s relay loan product refers to a personal housing loan that both a father (or mother) with full civil capacity and a son (or daughter) with full civil capacity apply to the bank as co-borrowers. This product adds children as co-borrowers, and calculates the loan period based on the age of the children (age + loan period not exceeding 70 years old), which effectively meets the reasonable housing loan demand of family members participating together, and effectively reduces the pressure of customers to repay. There is no situation where people over 70 years old can still get loans, which meets the requirements of supervision. \textcolor{blue}{NEI}\\
\midrule
\textbf{Gold}: 该产品通过增加子女作为共同借款人，并以子女年龄测算贷款期限（年龄+贷款期限不超过70岁），有效满足了家庭成员共同参与的合理住房贷款需求，有效降低了客户还款压力，不存在年龄超过70岁还能贷款的情形，符合监管的要求。记者向杭州多位银行一线业务人员求证，对方均表示暂未收到任何延长贷款人年龄的相关通知。By adding children as co-borrowers, and calculating the loan term based on the age of the children (age + loan term not exceeding 70 years old), this product effectively meets the reasonable housing loan demand of family members participating together, and effectively reduces the pressure of customers to repay. There is no situation where people over 70 years old can still get loans, which meets the requirements of supervision. The reporter asked many front-line business personnel in Hangzhou banks for verification, and they all said that they have not received any notice to extend the age of the lender. \textcolor{orange}{REF}\\
% \midrule
% \midrule
% \textbf{Claim 3}: 义乌市大数据机构神预测法国的黄马甲运动要蔓延。The big data agency of Yiwu City accurately predicted the spread of the yellow vest movement in France. \textcolor{orange}{REF}\\
% \midrule
% \textbf{JS}: 他告诉记者，今年下半年黄马甲的销量比上半年好一些，但还是比去年同期差，因为去年俄罗斯世界杯的举办推动了销量的上涨。从实际销量来看，张先生告诉记者，自己的企业今年对欧盟的马甲销售量和去年持平，而据他了解，今年整个武义县对欧的销售量是下滑的，完全没有新闻中说的“卖光”“脱销”“订单不断涌来”的情况。He told reporters that the yellow vest sales in the second half of this year were better than in the first half, but still worse than the same period last year, because last year's World Cup in Russia boosted sales. In terms of actual sales, Mr. Zhang told reporters that his company’s sales of vests to the EU this year were the same as last year. According to his understanding, the sales volume of Wuyi County to Europe has declined this year, and there is no such thing as ``sold out'', ``out of stock'' and ``continuous influx of orders'' mentioned in the news. \textcolor{blue}{NEI} \\
% \midrule
% \textbf{Gold}: 第一，从反光马甲行业的基本常识来看，绝大多数销往法国和其他欧盟国家的马甲一贯就不是从义乌市场上采购的，而是从和义乌同属于浙江省金华市的武义县采购。第二，从实际销量来看，张先生告诉记者，自己的企业今年对欧盟的马甲销售量和去年持平，而据他了解，今年整个武义对欧的销售量是下滑的，完全没有新闻中说的“卖光”“脱销”“订单不断涌来”的情况。第三，从张先生掌握的市场需求情况来看，以现在法国“黄马甲”运动这个规模，对马甲的需求量也只占平常法国总订单量中的很小一部分，即使中国这边的订单量出现什么变化，也完全不能由此得出结论“黄马甲运动要蔓延了”。First, from the basic knowledge of the reflective vest industry, the vast majority of vests sold to France and other EU countries have not always been purchased from the Yiwu market, but from Wuyi County, which belongs to Jinhua City, Zhejiang Province. Second, from the actual sales volume, Mr. Zhang told reporters that his company’s sales volume to EU vests this year was the same as last year. According to his understanding, the sales volume of Wuyi County to Europe has declined this year, and there is no such thing as ``sold out'', ``out of stock'' and ``continuous influx of orders'' mentioned in the news. Thirdly, from the market demand situation mastered by Mr. Zhang, with the current scale of the ``yellow vest'' movement in France, the demand for vests only accounts for a very small part of the usual total French orders. Even if there is any change in the order volume on China's side, it cannot be concluded that the ``yellow vest movement is about to spread.''.  \textcolor{orange}{REF}\\
% \textbf{Claim 1}: 突发头晕就是中风前兆。Sudden dizziness is a sign of stroke. \textcolor{orange}{REF}\\
% \midrule
% \textbf{Sem}: 其实脑血栓前期一般是有迹可循的，突发头晕就是中风前兆。In fact, the pre-cerebral thrombosis is generally traceable, and sudden dizziness is a precursor to stroke. \textcolor{green}{SUP}\\
% \midrule
% \textbf{JG}: 单纯的头晕症状无需与中风进行联系。The simple symptoms of dizziness do not need to be associated with a stroke. \textcolor{orange}{REF}\\
% \midrule
% \textbf{JS}: 头晕的原因非常多样，不一定是中风，但应及时就医排查。There are many causes of dizziness, not necessarily a stroke, but you should seek medical attention in time. \textcolor{blue}{NEI} \\
% \midrule
% \textbf{Gold}: 头晕是非常常见的神经内科疾病。单纯的头晕症状无需与中风进行联系。Dizziness is a very common neurological disease. Simple dizziness symptoms do not need to be connected with stroke. \textcolor{orange}{REF} \\
% \midrule
% \midrule
% \textbf{Claim 2}: 喝醋喝盐水不能消灭新冠病毒。Drinking vinegar and salt water can't eliminate the COVID-19. \textcolor{green}{SUP}\\
% \midrule
% \textbf{Sem}: 新冠病毒会在咽喉滞留4天，需要喝盐水和醋来消毒。The COVID-19 will stay in the throat for 4 days and need to drink salt water and vinegar to disinfect. \textcolor{orange}{REF}\\
% \midrule
% \textbf{JG}: 比病毒还可怕的科学流言：盐水漱口能预防新冠感染。A scientific rumor that is more terrifying than a virus: gargle with salt water can prevent the COVID-19 infection. \textcolor{green}{SUP}\\
% \midrule
% \textbf{JS}: 盐水和醋对病毒本身并没有作用。目前对新冠病毒有效的消毒方式有医用75\%酒精。Salt water and vinegar have no effect on the virus itself. At present, the effective disinfection method for the COVID-19 is medical 75\% alcohol. \textcolor{blue}{NEI} \\
% \midrule
% \textbf{Gold}: 盐水、醋和清水对新冠病毒本身并没有杀灭作用。Salt water, vinegar and clean water have no effect on the COVID-19 itself. \textcolor{green}{SUP} \\
\bottomrule
\end{tabularx}}
\vspace{-2mm}
\caption{Error analysis of the joint system. The evidence extracted by pipeline and joint systems based on the given claim is listed. The gold label of the claim and the veracity label based on the extracted evidence is highlighted.}
\label{tab:error_analysis}
% \vspace{-4mm}
\end{table*}
\end{CJK*}
